$(RSA)^2$: A Rhetorical-Strategy-Aware Rational Speech Act Framework for Figurative Language Understanding

Figurative language (e.g., irony, hyperbole, understatement) is ubiquitous in human communication, resulting in utterances where the literal and the intended meanings do not match. The Rational Speech Act (RSA) framework, which explicitly models speaker intentions, is the most widespread theory of probabilistic pragmatics, but existing implementations are either unable to account for figurative expressions or require modeling the implicit motivations for using figurative language (e.g., to express joy or annoyance) in a setting-specific way. In this paper, we introduce the Rhetorical-Strategy-Aware RSA $(RSA)^2$ framework which models figurative language use by considering a speaker's employed rhetorical strategy. We show that $(RSA)^2$ enables human-compatible interpretations of non-literal utterances without modeling a speaker's motivations for being non-literal. Combined with LLMs, it achieves state-of-the-art performance on the ironic split of PragMega+, a new irony interpretation dataset introduced in this study.

==> archived_versions/acl_submissions.tex <==
% Paragraph 1: Figurative uses of language are ubiquitous/critical part of human communication. Provide some examples - use a weather example to prepare the reader for the running example.

% Paragraph 2: At the same time, LLMs, which have become the primary way of interfacing with language technologies, have been shown to perform poorly on figurative language interpretation. Figure 1 shows an example. List some reasons for why this might be (use the wording that Jackie suggested), guide the reader to implying that it's due to a lack of explicitly reasoning about the rhetorical strategy being used.

% Segue from LLM to this paragraph with communicative goal, this allows you to talk about RSA and then to talk about affect-aware RSA
Paragraph 3: This failure of LLMs suggests that their inference procedure should reason more explicitly about a speaker's choice of rhetorical strategy when interpreting an utterance. Use the weather example to make this more concrete. [Jackie: Use communicative goal to make the segue smoother and less about comparing with affect-aware RSA.]

Paragraph 4: It turns out that there already exists a model of human communication which makes these reasoning steps explicit: RSA. Briefly describe the general idea behind RSA and how, in its original formulation, it is unsuitable for non-literal language (Add a reference to where we prove this more formally). As a result, affect-aware RSA has been proposed to mitigate this problem but makes the assumption that figurative language's primary use is to convey affect and/or valence even though it's been shown to be used for other things (e.g. criticizing, softening, etc.). Refer to related work for a more detailed discussion.

While affect-aware RSA is successful in enabling the RSA framework to obtain non-literal interpretations of utterances, it results in a framework which we believe does not faithfully reflect the communicative goal of utterances employed a figurative manner. As a result of coupling non-literal meaning with affect, the framework is unable to account for figurative uses of language which are not affect-driven for instance, in conventionalized language \citep{ContextualEffectsUnderstanding1979}. For example, the exaggeration in the phrase ``The weather here is always terrible'' might be meant to describe how often bad weather occurs, rather than to express the speaker's feelings about it.

Paragraph 5: As a result, we introduce \rsatwospace where a speaker's rhetorical strategy is explicitly modeled and used to adjust listener expectations. \rsatwospace shifts the belief distribution of a listener based on the rhetorical strategy (define rhetorical strategy formally here) to enable non-literal interpretations of utterances *without* having to assume any particular speaker affect. The rhetorical strategy can either be set explicitly like in our weather example, a practice (the hardcoding of things) commonly followed in cognitive science studies which use RSA to predict the utterance or meaning of a human generated utterance in a specific scenario or it can be inferred by considering the difference in intended meaning between the utterance being interpreted and alternative utterances which may have been generated in the same context.

Paragraph 6: List some of the main results: In section 3, we provide a toy experiment where we illustrate how, by explicitly considering a speaker's rhetorical strategy, we are able to handle several different figurative uses of language as they pertain to describe the weather: irony, hyperbole, understatement which the original and affect-aware RSA formulations could not handle. In section 4, we show how a listener's expectations may be adjusted automatically at inference by inferring rhetorical strategy adjustment coefficients and provide a concrete implementation using LLMs in section 5. We show that \rsatwospace enables LLM's to shift their probability distribution of the meanings of an utterance which aligns with rhetorical strategy being used. Concretely, use and expand the PragMega dataset and show X performance gains.

Paragraph 7: List core contributions: 1. We provide an alternative formulation to RSA which can handle figurative uses of language by explicitly reasoning about the employed rhetorical strategy. 2. We show that our method enables LLMs to provide more faithful interpretations of figurative uses of language.

By modeling communication in this manner, the RSA framework has been shown to successfully predict the meaning of literally ambiguous utterances such as ``some'' in scalar implicatures. However, it can be shown that interpretations of utterances which are not compatible with the literal meaning of an utterance will be assigned zero probability by the pragmatic listener (Proof in Appendix~\ref{app:rsa_theory}). That is, in the standard RSA framework, the only meanings of ``This one is really sharp.'' from  Figure~\ref{fig:john-example} which could receive non-zero probability would be ones which are semantically entailed by this utterance, namely that the student is in fact smart when the context suggests they are not.

As a result, efforts to model human use of figurative language have sought to address this limitation by incorporating the affect of an utterance within the RSA framework. As described in Section~\ref{}, the authors enable non-literal meanings to receive probability mass from the pragmatic listener by coupling an utterance's meaning and affect together. For instance, in our earlier example, a pragmatic listener may interpret the utterance ``It is so nice outside.'' in the context of a snowstorm as meaning that the weather is bad because this meaning is typically associated with a negative affect (e.g., annoyance or frustration).

While affect-aware RSA is successful in enabling the RSA framework to obtain non-literal interpretations of utterances, it results in a framework which we believe too tightly couples the notion of non-literal meaning and affect. As a result of this coupling, the framework is unable to account for figurative uses of language which are not affect-driven \citep{ContextualEffectsUnderstanding1979}. For example, in Figure~\ref{fig:john-example}, it is not clear that the John's ironic utterance ``This one is really sharp.'' is meant to convey affect. Instead, John may simply be used to conveying information about students' academic performances in a non-literal manner. Rather than pinpointing the exact --- if at all present --- affect which motivated the speaker's figurative use of an utterance, we believe that reasoning about the employed non-literal rhetorical strategy is a more direct way of enabling RSA to produce non-literal meaning interpretations of utterances.

By introducing a rhetorical strategy prior along with an adaptable semantic understanding function $\llbracket \cdot \rrbracket_r$, we are able to modify which meaning interpretations receive probability mass from the literal listener and, thus, which meanings will be available to the pragmatic listener when applying its Bayesian posterior update. For instance, under $r = \text{literal}$, $\texttt{The student is not clever.} \notin \llbracket \text{``This one is really sharp.''} \rrbracket^r$, while for $r = \text{ironic}$ $\texttt{The student is not clever.} \in \llbracket \text{``This one is really sharp.''} \rrbracket^r$. The pragmatic listeners under each rhetorical strategy are then marginalized together to produce a rhetorical-stategy-aware meaning interpretation of the utterance $u$, $P_{L_1}(m|c,u)$.

We test our formulation on the same setting as \citet{Kao2015Irony} which proposed an affect-aware RSA formulation to interpret utterances describing the weather. In this setting, the possible intended meanings included describing the weather as \texttt{terrible}, \texttt{bad}, \texttt{ok}, \texttt{good} or \texttt{amazing}. The set of possible utterances included all utterances of the form ``The weather is $x$'' where $x$ was one of the aforementioned intended meanings. Finally, these utterances and meanings were communicated under two contexts: one where the weather is sunny with clear skies and another with heavy precipitation (e.g., rain or snow) and winds.

==> archived_versions/extra_notes.tex <==
% Paragraph 1: Figurative uses of language are ubiquitous/critical part of human communication. Provide some examples - use a weather example to prepare the reader for the running example.

% Paragraph 2: At the same time, LLMs, which have become the primary way of interfacing with language technologies, have been shown to perform poorly on figurative language interpretation. Figure 1 shows an example. List some reasons for why this might be (use the wording that Jackie suggested), guide the reader to implying that it's due to a lack of explicitly reasoning about the rhetorical strategy being used.

% Segue from LLM to this paragraph with communicative goal, this allows you to talk about RSA and then to talk about affect-aware RSA
Paragraph 3: This failure of LLMs suggests that their inference procedure should reason more explicitly about a speaker's choice of rhetorical strategy when interpreting an utterance. Use the weather example to make this more concrete. [Jackie: Use communicative goal to make the segue smoother and less about comparing with affect-aware RSA.]

Paragraph 4: It turns out that there already exists a model of human communication which makes these reasoning steps explicit: RSA. Briefly describe the general idea behind RSA and how, in its original formulation, it is unsuitable for non-literal language (Add a reference to where we prove this more formally). As a result, affect-aware RSA has been proposed to mitigate this problem but makes the assumption that figurative language's primary use is to convey affect and/or valence even though it's been shown to be used for other things (e.g. criticizing, softening, etc.). Refer to related work for a more detailed discussion.

While affect-aware RSA is successful in enabling the RSA framework to obtain non-literal interpretations of utterances, it results in a framework which we believe does not faithfully reflect the communicative goal of utterances employed a figurative manner. As a result of coupling non-literal meaning with affect, the framework is unable to account for figurative uses of language which are not affect-driven for instance, in conventionalized language \citep{ContextualEffectsUnderstanding1979}. For example, the exaggeration in the phrase ``The weather here is always terrible'' might be meant to describe how often bad weather occurs, rather than to express the speaker's feelings about it.

Paragraph 5: As a result, we introduce \rsatwospace where a speaker's rhetorical strategy is explicitly modeled and used to adjust listener expectations. \rsatwospace shifts the belief distribution of a listener based on the rhetorical strategy (define rhetorical strategy formally here) to enable non-literal interpretations of utterances *without* having to assume any particular speaker affect. The rhetorical strategy can either be set explicitly like in our weather example, a practice (the hardcoding of things) commonly followed in cognitive science studies which use RSA to predict the utterance or meaning of a human generated utterance in a specific scenario or it can be inferred by considering the difference in intended meaning between the utterance being interpreted and alternative utterances which may have been generated in the same context.

Paragraph 6: List some of the main results: In section 3, we provide a toy experiment where we illustrate how, by explicitly considering a speaker's rhetorical strategy, we are able to handle several different figurative uses of language as they pertain to describe the weather: irony, hyperbole, understatement which the original and affect-aware RSA formulations could not handle. In section 4, we show how a listener's expectations may be adjusted automatically at inference by inferring rhetorical strategy adjustment coefficients and provide a concrete implementation using LLMs in section 5. We show that \rsatwospace enables LLM's to shift their probability distribution of the meanings of an utterance which aligns with rhetorical strategy being used. Concretely, use and expand the PragMega dataset and show X performance gains.

Paragraph 7: List core contributions: 1. We provide an alternative formulation to RSA which can handle figurative uses of language by explicitly reasoning about the employed rhetorical strategy. 2. We show that our method enables LLMs to provide more faithful interpretations of figurative uses of language.

By modeling communication in this manner, the RSA framework has been shown to successfully predict the meaning of literally ambiguous utterances such as ``some'' in scalar implicatures. However, it can be shown that interpretations of utterances which are not compatible with the literal meaning of an utterance will be assigned zero probability by the pragmatic listener (Proof in Appendix~\ref{app:rsa_theory}). That is, in the standard RSA framework, the only meanings of ``This one is really sharp.'' from  Figure~\ref{fig:john-example} which could receive non-zero probability would be ones which are semantically entailed by this utterance, namely that the student is in fact smart when the context suggests they are not.

As a result, efforts to model human use of figurative language have sought to address this limitation by incorporating the affect of an utterance within the RSA framework. As described in Section~\ref{}, the authors enable non-literal meanings to receive probability mass from the pragmatic listener by coupling an utterance's meaning and affect together. For instance, in our earlier example, a pragmatic listener may interpret the utterance ``It is so nice outside.'' in the context of a snowstorm as meaning that the weather is bad because this meaning is typically associated with a negative affect (e.g., annoyance or frustration).

While affect-aware RSA is successful in enabling the RSA framework to obtain non-literal interpretations of utterances, it results in a framework which we believe too tightly couples the notion of non-literal meaning and affect. As a result of this coupling, the framework is unable to account for figurative uses of language which are not affect-driven \citep{ContextualEffectsUnderstanding1979}. For example, in Figure~\ref{fig:john-example}, it is not clear that the John's ironic utterance ``This one is really sharp.'' is meant to convey affect. Instead, John may simply be used to conveying information about students' academic performances in a non-literal manner. Rather than pinpointing the exact --- if at all present --- affect which motivated the speaker's figurative use of an utterance, we believe that reasoning about the employed non-literal rhetorical strategy is a more direct way of enabling RSA to produce non-literal meaning interpretations of utterances.

By introducing a rhetorical strategy prior along with an adaptable semantic understanding function $\llbracket \cdot \rrbracket_r$, we are able to modify which meaning interpretations receive probability mass from the literal listener and, thus, which meanings will be available to the pragmatic listener when applying its Bayesian posterior update. For instance, under $r = \text{literal}$, $\texttt{The student is not clever.} \notin \llbracket \text{``This one is really sharp.''} \rrbracket^r$, while for $r = \text{ironic}$ $\texttt{The student is not clever.} \in \llbracket \text{``This one is really sharp.''} \rrbracket^r$. The pragmatic listeners under each rhetorical strategy are then marginalized together to produce a rhetorical-stategy-aware meaning interpretation of the utterance $u$, $P_{L_1}(m|c,u)$.

We test our formulation on the same setting as \citet{Kao2015Irony} which proposed an affect-aware RSA formulation to interpret utterances describing the weather. In this setting, the possible intended meanings included describing the weather as \texttt{terrible}, \texttt{bad}, \texttt{ok}, \texttt{good} or \texttt{amazing}. The set of possible utterances included all utterances of the form ``The weather is $x$'' where $x$ was one of the aforementioned intended meanings. Finally, these utterances and meanings were communicated under two contexts: one where the weather is sunny with clear skies and another with heavy precipitation (e.g., rain or snow) and winds.
